Factuality of Large Language Models: A Survey

Large language models (LLMs), especially when instruction-tuned for chat, have become part of our daily lives, freeing people from the process of searching, extracting, and integrating information from multiple sources by offering a straightforward answer to a variety of questions in a single place. Unfortunately, in many cases, LLM responses are factually incorrect, which limits their applicability in real-world scenarios. As a result, research on evaluating and improving the factuality of LLMs has attracted a lot of attention recently. In this survey, we critically analyze existing work with the aim to identify the major challenges and their associated causes, pointing out to potential solutions for improving the factuality of LLMs, and analyzing the obstacles to automated factuality evaluation for open-ended text generation. We further offer an outlook on where future research should go.

==> assets/outline.tex <==
% https://ijcai24.org/call-for-papers-survey-track/
% How Should the Paper Be Written?
% The survey should have a well-defined scope and be understandable for most of the AI community. It should clarify why the topic is important and its intended or existing applications. The survey should be comprehensive concerning state of the art, with a personal stance on the topic: the description of the existing work should be structured. It should contain a discussion (aiming, for instance, at comparing alternative approaches or identifying open questions and challenges). It should not be a simple juxtaposition of summaries of papers or groups of papers. While the authors’ work can sometimes be an important part of a survey, there should be no significant bias towards it: the work of others should be mentioned and appreciated by its relevance and importance. The paper should be of very high quality in terms of presentation, be at the appropriate technical level, and be grounded in the existing literature.

% length: 7 + 2

==> section/dataset.tex <==
\subsection{Datasets}
\label{sec:datasets}
% Jiahui

Snowballing dataset~\cite{zhang2023snowball} comprises three question-answering subsets: primality testing, senator search and graph connectivity, each with 500 yes/no questions.
They aim to investigate snowballing hallucination when model immediately output an incorrect answer (yes or no) as false generated context. Specifically, they prompt language model to first output yes/no answer and then provide explanations.
When the immediate answer is wrong, the model tends to continue to snowball the false statements instead of correcting it.
% The Flights dataset always yields 'no' answers, as it lacks a sequence of connecting flights. In the Prime dataset, answers are consistently 'yes,' with all numbers being prime. Lastly, the Senator dataset invariably provides 'no' answers, as no senator meets both specified criteria: originating from a particular state and attending a certain college.
% 
CoVe used four datasets~\cite{dhuliawala2023chain}.
One is selected from Wikidata --- listing of people with specific professions born in a certain city (56 questions), and the other is listing works from specific categories based on Wiki-category (55 questions), e.g., \textit{Name some Mexican animated horror films or Name some Endemic orchids of Vietnam}.
The third dataset consists of 418 questions sampled from the MultiSpanQA test set with shorter answers per span (up to 3 tokens per item).
They also apply the dataset of generating biographies as FactScore.

% However, they do not release their datasets and code for reproduction.
% We try to collect similar datasets. It is non-trivial due to the subjective selection.
% The second and the third might be possible but is not worthwhile to spend the time on collecting such data.



TruthfulQA~\cite{lin-etal-2022-truthfulqa} is a benchmark designed to measure whether a language model is truthful in generating answers to questions and is robustness on false belief or misconception. It comprises 817 questions spanning 38 categories, including health, law, finance, and politics. The dataset includes both text generation and multiple-choice components, with the multiple-choice questions having a variable number of options. The questions are designed to be "adversarial" to test for weaknesses in the truthfulness of language models rather than testing models on a useful task.

HELM~\cite{liang2023holistic} is a living benchmark designed to enhance the transparency of language models. The dataset implements a multi-metric approach, encompassing various user-facing tasks, domains, and languages. It includes a core set of scenarios and metrics, covering tasks such as question answering, information retrieval, summarization, and toxicity detection across different domains and languages. The dataset is intended to be continuously updated with new scenarios, metrics, and models, and all raw model prompts and completions are released publicly for further analysis. 

FacTool~\cite{chern2023factool} detected factual errors in LLM generations across four different tasks: knowledge-based QA, code generation, mathematical reasoning, and scientific literature review. During model evaluation, they reported both response-level and claim-level accuracy when the responses consist of several claims.

Factcheck-GPT~\citep{wang2023factcheck} Factcheck-GPT gathered a total of 94 highly challenging questions from sources including Twitter posts, internal brainstorming, and Dolly-15k, encompassing 678 claims.

HaluEval~\cite{li2023halueval} comprises 5,000 general user queries accompanied by ChatGPT responses and 30,000 specialized examples from three distinct tasks: question answering, knowledge-grounded dialogue, and text summarization.

FreshQA~\cite{vu2023freshllms} is composed of 600 natural, open-ended questions, segmented into four primary categories based on the answer's stability: 'never-changing' for answers that rarely alter; 'slow-changing' for those that evolve over several years; 'fast-changing' for answers that shift within a year or less; and 'false-premise', encompassing questions with factually incorrect premises that need to be countered.

Self-Aware~\cite{yin-etal-2023-large} compiled a collection of 1,032 unanswerable questions from online platforms like Quora and HowStuffWorks. In addition, they gathered a total of 2,337 answerable questions from sources such as SQuAD, HotpotQA, and TriviaQA.

FACTOR~\cite{muhlgay2023factor} introduces a framework automatically transforms a factual corpus of interest into a benchmark for evaluating an LM's creates factuality, and creating two benchmarks using this framework: Wiki-FACTOR and News-FACTOR. Wiki-FACTOR is based on the Wikipedia section of The Pile's validation split and consists of 2994 examples, while News-FACTOR is based on Reuters articles extracted from The RefinedWeb Dataset and consists of 1036 examples. 

% Adding FELM
FELM~\cite{chen2023felm} introduces a benchmark for Factuality Evaluation of large Language Models,
referred to as FELM. This benchmark collects responses generated from LLMs and annotate factuality labels in a fine-grained manner. The related dataset consists of 5 categories, with examples per category as follows - 194 math, 208 reasoning, 125 science, 184 world knowledge (wk) and 136 writing recordings.

% Additionally, introduces Expert-FACTOR, which is based on the validation and test splits of ExpertQA, a long-form question-answering dataset, and consists of 236 examples. 

Self-Contradictory~\cite{anonymous2023selfcontradictory} constructed a dataset by sampling language model responses about various topics, consisting of 360 text descriptions covering 30 diverse topics.

SelfCheckGPT~\cite{manakul2023selfcheckgpt} generated synthetic Wikipedia articles on individuals/concepts from the WikiBio dataset~\cite{lebret2016generating} using GPT-3, followed by manual annotation to assess the factuality of each passage at the sentence level. 

FactScore~\cite{min2023factscore} utilized a total of 13 language models and prompted these models to generate biographies of 500 individuals, resulting in a total of 6,500 generations.


==> section/factual_error_rate_table.tex <==
% To-do (Minghan)
% Add a table to statitically list percentage of false and true claims for ChatGPT (several human labelled dataset)
% Add factuality score of some models under the same evaluation benchmark, such as MMLU, TruthfulQA and hallucination-index

Evaluation tables: 
Table 1: Human annotation for ChatGPT factuality score over several labeled benchmark
Table 2：frequently-used datasets in leaderboard + hallucination index on various LLMs factuality score
Table 3: Examples for four types of dataset instance

Abstract:
Large language models (LLMs), especially when instruction-tuned for chat, have become part of our daily lives, freeing people from the process of searching, extracting, and integrating information from multiple sources by offering a straightforward answer to a variety of questions in a single place. Unfortunately, in many cases, LLM responses are factually incorrect, which limits their applicability in real-world scenarios. As a result, research on evaluating and improving the factuality of LLMs has attracted a lot of research attention recently. In this survey, we critically analyze existing work with the aim to identify the major challenges and their associated causes, pointing out to potential solutions for improving the factuality of LLMs, and analyzing the obstacles to automated factuality evaluation for open-ended text generation. We further offer an outlook on where future research should go.

@article{geva2021strategyqa,
  title={Did aristotle use a laptop? a question answering benchmark with implicit reasoning strategies},
  author={Geva, Mor and Khashabi, Daniel and Segal, Elad and Khot, Tushar and Roth, Dan and Berant, Jonathan},
  journal={Transactions of the Association for Computational Linguistics},
  volume={9},
  pages={346--361},
  year={2021},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}
